Knowledge Generation for Zero-shot Knowledge-based VQA

Previous solutions to knowledge-based visual question answering~(K-VQA) retrieve knowledge from external knowledge bases and use supervised learning to train the K-VQA model. Recently pre-trained LLMs have been used as both a knowledge source and a zero-shot QA model for K-VQA and demonstrated promising results. However, these recent methods do not explicitly show the knowledge needed to answer the questions and thus lack interpretability. Inspired by recent work on knowledge generation from LLMs for text-based QA, in this work we propose and test a similar knowledge-generation-based K-VQA method, which first generates knowledge from an LLM and then incorporates the generated knowledge for K-VQA in a zero-shot manner. We evaluate our method on two K-VQA benchmarks and found that our method performs better than previous zero-shot K-VQA methods and our generated knowledge is generally relevant and helpful.

==> sections/experiment_v1.tex <==
\section{Experiments}
% \label{sec:exp}

\subsection{Datasets}
To validate our proposed method, we choose two commonly used K-VQA benchmark datasets, namely, OK-VQA~\cite{DBLP:conf/cvpr/MarinoRFM19} and A-OKVQA~\cite{DBLP:conf/eccv/SchwenkKCMM22}. 
Questions in OK-VQA need outside knowledge beyond the images to answer.
% and cannot be obtained with a few knowledge bases.
A-OKVQA is an augmented version of OK-VQA that requires additional types of world knowledge to answer.
Because the ground-truth answers of the \textit{test-split} of A-OKVQA are not available, we use the \textit{val-split} of A-OKVQA for evaluation. 
OK-VQA and A-OKVQA contains $5,046$ test questions and $1,100$ validation questions.

\subsection{Implementation Details}
For knowledge generation, we prompt the large langauge model (LLM), \textit{text-davinci-003}\footnote{https://platform.openai.com/docs/models/gpt-3-5} with the OpenAI API, with a suggested temperature of $0.7$. We use BLIP model~\cite{DBLP:conf/icml/0001LXH22} to convert images into textual descriptions and we adopt the question-aware caption generation similar to~\cite{DBLP:journals/corr/abs-2212-10846,DBLP:conf/emnlp/Tiong0LSH22}.
For each testing question, we use $65$ pieces of generated image captions and $10$ pieces of generated knowledge as the contexts with a trade-off between the computational cost and performances. We use the Fusion-in-Decoder~\cite{DBLP:conf/eacl/IzacardG21} with the UnifiedQA~\cite{DBLP:conf/emnlp/KhashabiMKSTCH20} checkpoint as our QA model for reporting results. We also test other QA models, such as the fusion-in-encoder T5 model~\cite{DBLP:conf/emnlp/KhashabiMKSTCH20} and GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20} and more results are provided in Section~\ref{sec:ablations}. 
   



\begin{table}[t]
\centering
\begin{small}
  \begin{tabular}{l|ccc}
    \toprule
    \textbf{QA Model}&\textbf{Num.} & \textbf{OK-VQA} & \textbf{A-OKVQA}\\
    \midrule\multirow{4}{*}{FiE-T5\footnote{For FiE-T5 model, we are unable to use as many captions as the FiD-T5 model due to high computational cost. Instead we leverage LLaVA for generating one detailed question-related image captions.} }&
    0 & 28.1&  33.7\\
    &5 &30.7 & 28.4 \\
    &10& 31.8&28.0  \\
    &20 &32.8 & 27.4 \\
    \midrule\multirow{4}{*}{GPT-3}&
    0 & 27.4&  -\\
    &5 & 34.1&  -\\
    & 10 & 32.4& - \\
    &20 &31.7 &  -\\
    \midrule
    \multirow{4}{*}{FiD-T5}&
    0 & 34.1&  35.5\\
    &5 & 40.9&  36.5\\
    &10 & 41.1&  35.2\\
    &20 &39.7 & 33.8 \\
   % &25 &39.2 &  \\
    \midrule
\end{tabular}
\end{small}
\caption{Performances of our method with different number of generated knowledge pieces.}
  \label{tab:num-kb-past}
\end{table}

\begin{table}[t]
\centering
\begin{small}
  \begin{tabular}{l|cc}
    \toprule
    \textbf{Case}&\textbf{Num. Kn.} & \textbf{OK-VQA} \\
    \midrule
    Manual &1 &38.6  \\
    Cluster &1 & 39.7\\
    Random\footnote{Due to the cost of GPT-3, for random demonstration selection, we only validate the performance on a subset of the testing data. Our cluster-based selection got 40.1 on the subset OK-VQA.} & 10& 38.6\\
    Cluster &10 &41.1 \\
    \midrule
\end{tabular}
\end{small}
\caption{The impact of the cluster-based knowledge generation.}
  \label{tab:cluster-kb}
\end{table}

\subsection{Baselines}
We categorize the compared zero-shot K-VQA models into three types: 1) zero-shot KB-VQA models without any more training; 2) zero-shot KB-VQA models but requiring extra training with other data, such as VL-T5~\cite{DBLP:conf/icml/ChoLTB21}, Frozen~\cite{DBLP:conf/nips/TsimpoukelliMCE21}, VLKD~\cite{DBLP:conf/acl/DaiHSJLF22}, FewVLM~\cite{DBLP:conf/acl/Jin0SC022}, BLIP-2~\cite{DBLP:journals/corr/abs-2301-12597} and Flamingo~\cite{DBLP:conf/nips/AlayracDLMBHLMM22}; 3) models requiring few training examples (with or without extra training), such as PICa in few-shot learning setting (PICa$_\text{few}$)~\cite{DBLP:conf/aaai/YangGW0L0W22} and PromptCap~\cite{DBLP:journals/corr/abs-2211-09699,DBLP:conf/aaai/YangGW0L0W22}. We provide a brief overview of three kinds of models in Table~\ref{tab:model-info}. In this study, we intent to compare with zero-shot K-VQA models in similar model scales without extra training (i.e., models in the first block). Below we briefly introduce models in the first block.

PICa~\cite{DBLP:conf/aaai/YangGW0L0W22} converted images of K-VQA into textual descriptions so that K-VQA is converted into text-based question answering and prompted GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20} together with the question for answer prediction. PNP-VQA~\cite{DBLP:conf/emnlp/Tiong0LSH22} generated question-aware image descriptions and prompt a pre-trained unified question answering model~\cite{DBLP:conf/emnlp/KhashabiMKSTCH20} for answers. Img2LLM~\cite{DBLP:journals/corr/abs-2212-10846} followed a similar process of PICa but generate synthetic question-answer pairs according to the image and the synthetic QA pairs will sever as examples when prompting LLMs (e.g., GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20} and OPT~\cite{DBLP:journals/corr/abs-2205-01068}).
%\crtext{consider models of similar model scales. models with larger model sizes provided in appendix; but for PICa and BLIP-2, how to jjustify the results}

\subsection{Main Results}
Here we provide the main experimental results on OK-VQA and A-OKVQA in Table~\ref{tab:results-okvqa} and Table~\ref{tab:results-aokvqa} respectively. \crcomment{shall we mention few-shot learning models (e.g., PICa and PromptCap) sampled over the whole dataset}

\subsection{Ablation Study}
\label{sec:ablations}
\noindent\textbf{Number of Augmented Knowledge Pieces}

\noindent\textbf{Cluster-based Generated Knowledge} in Tavble~\ref{tab:cluster-kb}.

\noindent\textbf{Different Question Answering Models}
%GPT-3
%FiD
%T5

\noindent\textbf{Different Captions:} We also test the robustness of our method with different captions in terms of different caption generators and different number of captions.

\subsection{Human Evaluation}
%how to choose cases
In this section, we conduct human evaluation to exam the quality of the generated knowledge. We follow~\cite{DBLP:conf/acl/0010LLWWBCH22} and sample $40$ cases the correctness of which would be changed (i.e., either from correct to wrong or wrong to correct) after augmenting knowledge from OK-VQA dataset. For each instance, we sample $5$ pieces of generated knowledge which has been used for K-VQA for evaluation. We ask two annotators to check the quality of the generated knowledge in terms of evaluation metrics below. To ensure objectiveness, annotators will not know whether the predictions are changed correct or wrong. We provide the files assigned to annotators (including task instruction, evaluation guidance and examples for evaluation) and the evaluation results from annotators in the supplementary folder.

\noindent\textbf{Evaluation Metrics} Following~\cite{DBLP:conf/acl/0010LLWWBCH22,DBLP:conf/emnlp/ShwartzWBBC20}, we take four metrics for evaluating generated knowledge: 1) \textit{Grammatically}: whether the it is grammatical  2) \textit{Relevance}: whether it is related to answering the question and the image; 3) \textit{Factuality}: whether it is factual; 4) \textit{Helpfulness}: whether it is helpful so that it directly leads to the correct answers or provides indirect but supportive information of the correct answers. For \textit{helpfulness}, we adopt three categories of evaluation: helpful (i.e.., provides direct or indirect supportive information to correct answers), harmful (i.e., negates correct answers or support incorrect answers) or neutral (neither helpful or harmful). Details about the definitions can be found in Appendix~\ref{sec:human-eval-details} and the examples we provided to annotators regarding the four evaluation metrics are included in Supplementary. 

\noindent\textbf{Chain-of-Thought Generate Knowledge} The idea of Chain-of-Thoughts (CoT) has been widely adopted as ~\cite{DBLP:conf/nips/Wei0SBIXCLZ22}, which generates explanations before the answer generation. In K-VQA, the needed knowledge can also be regarded as a kind of explanations. Therefore, we test the widely used CoT for knowledge generation, which is alternative to our cluster-based knowledge generation approach. We re-use the eight manual demonstrations as mentioned in Section~\ref{sec:method} and manually add answers to the questions (i.e., each demonstration will consist of contexts of image descriptions, a question, a piece of related knowledge and an answer). Together with these demonstrations, we prompt GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20} to first generate the relevant knowledge and then the answer. Due to the cost of calling GPT APIs, we only apply CoT to a subset questions on OK-VQA (200 questions).

\noindent\textbf{Results} The average agreement from two annotators over four evaluation metrics is $0.67$, in terms of \textit{Fleiss Kappa} $\kappa$~\cite{landis1977measurement}. It indicates substantial agreement among annotators. For each criteria, we report the average score over two annotators.
Besides the interpretability of generated knowledge, we also think of comparing the K-VQA performance when augmenting with two alternative ways of generating knowledge. Firstly, we directly compared the CoT generated answer from GPT-3 after knowledge generation with prompting GPT-3 for QA with our generated knowledge together with image captions and questions. According to the table, we observe our approach prompting GPt-3 in two stages outperforming the CoT method, indicating that the cluster-based method may generated more diverse knowledge which facilitates K-VQA. Meanwhile, we consider the fact that exact match may be too strict as some GPT-3 answers are reasonable 

\subsection{Case Study}

\subsection{Error Analysis}

==> sections/intro_v1.tex <==
\section{Introduction (v1)}

Compared with the standard visual question answering (VQA) task~\cite{DBLP:journals/ijcv/AgrawalLAMZPB17}, the task of knowledge-based visual question answering (KB-VQA)~\cite{DBLP:journals/pami/WangWSDH18,DBLP:conf/cvpr/MarinoRFM19,DBLP:conf/eccv/SchwenkKCMM22} is more knowledge-intensive. Given an image and the corresponding image, KB-VQA required external knowledge beyond the image to answer the question. For instance, to answer the question in Figure~\ref{fig:intro-img}, the background knowledge about national parks in California is needed. Therefore, one key challenge in KB-VQA is how to obtain needed external knowledge.


%limitation (first): train a retriever; dis-match of knowledge bases and needed knowledge outside knowledge bases
A line of works propose a \textit{retrieve and answer} method~\cite{DBLP:conf/emnlp/GarderesZAL20,DBLP:conf/aaai/WuLSM22,DBLP:conf/mm/Li0020} (as illustrated in the Figure~\ref{fig:intro-img} (a)). They first retrieve knowledge from existing knowledge bases, such as Wikipedia, DBPedia~\cite{DBLP:conf/semweb/AuerBKLCI07} and ConceptNet~\cite{DBLP:conf/aaai/SpeerCH17} to retrieve relevant knowledge, by linking the question and the image representations to entities in knowledge bases. Then the retrieved knowledge will be integrated in the VQA stage with the question and the image. 
These retrieval based methods suffer from three limitations. 
Firstly, to retrieve relevant documents from knowledge bases, all documents should be encoded and the representations for each question-image pair should be stored, which is computationally expensive and limits the dimension of representations so that is hard to scale up with large models with high representation dimensions.
Secondly, the representations for questions and images in the retrieval stage and the VQA stage are trained independently, which may lead to mis-match between the retrieved knowledge and the knowledge in need.
Besides, one or a few knowledge bases may not cover knowledge for all knowledge-intensive questions~\cite{DBLP:conf/eccv/SchwenkKCMM22,DBLP:conf/cvpr/MarinoRFM19}.
\jjcomment{I am thinking that we may not want to talk too much about the disadvantages of methods that retrieve knowledge from KBs, especially if our method is not designed to address these limitations of previous methods. If we do so here, there may be the expectation for us to compare with these methods in terms of the considerations we mentioned. E.g., if we claim that these methods are computationally more expensive, then do we need to demonstrate in our experiments that our method are more efficient? (I don't think we intend to do that.) And if we claim that the retrieved knowledge by these methods may not be the most relevant, we may also need to show that our method generates better knowledge than these methods. (Again, I don't think we intend to do this.)} \crtext{Agree and I do not intent to do it neither.}



%why explicit: explanability
The other link of works try to leverage Large Language Models (LLMs) (e.e., T5~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20} and GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20}) as implicit knowledge bases~\cite{DBLP:conf/aaai/YangGW0L0W22,DBLP:conf/emnlp/Tiong0LSH22,DBLP:journals/corr/abs-2211-09699} through \textit{ask and answer} (as illustrated in the Figure~\ref{fig:intro-img} (b)). 
\jjcomment{Is the term ``ask and answer'' coined by some previous paper? The term itself does not sound very informative to me, because for VQA there is obviously ``ask'' and ``answer''. Maybe I can read the paper that coined the term and see why they proposed this term.} \crtext{No, I used the term myself, because this kind of methods ask QA models and use implicit knowledge in LMs to answer the question. This is in parallel with the \textit{retrieve and answer} above.}
As LLMs are unable to receive multimodal inputs, they will first convert images into textual descriptions. The image descriptions will serve as contexts and will be used together with questions to prompt LLMs in a question answering (QA) manner to obtain the prediction. However, it is unclear how LLMs give predictions and what external knowledge inside LLMs is used for QA. On the  other hand, a recent study showed that using explicitly generated knowledge LLMs can facilitate QA performances~\cite{DBLP:conf/acl/0010LLWWBCH22}. 
\jjcomment{We may want to think more carefully about how we should introduce the idea of generating knowledge explicitly. Right now this idea is somehow buried in this paragraph; it does not stand out. I feel we need to further emphasize this idea.}
In this work, we study whether we can similarly generate knowledge from LLMs for KB-VQA and whether such explicitly generated knowledge could improve the QA performance in the knowledge-intensive multimodal setting. To the best of our knowledge, we are the first that explicitly leverage knowlege from LLMs for KB-VQA.

We propose to prompt the frozen LLMs, such as GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20} to generate explicit related knowledge in KB-VQA. To make images understandable to LLMs, we convert images into their textual descriptions with the off-the-shelf caption generator. Then we prompt LLMs with using the question, the image description and an instruction asking LLMs for generating related knowledge for answering the question. 
%\crcomment{shall we state our prompt is conducted in a few-shot manner in the introduction part?}
To utilize the generated knowledge, we regard both the image descriptions and the knowledge as contexts and prompt a frozen text-based QA model with the question. 

We test the effectiveness of the proposed method on two KB-VQA datsaets~\cite{DBLP:conf/eccv/SchwenkKCMM22,DBLP:conf/cvpr/MarinoRFM19}. Besides the higher interpretability, our approach that explicitly generates knowledge from LLMs significantly outperforms those KB-VQA models using implicit knowledge in LLMs only and directly asking LLMs for answer generation (about $\mathbf{xxx\%}$ of absolute performance improvement over~\cite{DBLP:conf/emnlp/Tiong0LSH22} 3B model).
Besides, we validate our method with different text-based QA models (e.g., UnifiedQA~\cite{DBLP:conf/emnlp/KhashabiMKSTCH20}, FiD~\cite{DBLP:conf/eacl/IzacardG21} and GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20}). The improvements are consistent and obvious with different text-based QA models before and after inserting the generated background knowledge. We further conduct detailed analysis about the generated knowledge to prove it is essential and faithful.

Overall, we summarize our contributions as follows:

\begin{enumerate}
\item Rather than retrieving knowledge from existing knowledge bases or using implicit knowledge embedded in LLMs, we are the first to propose to explicitly generate knowledge with LLMs to help with the task of KB-VQA.
\item We integrate the generated knowledge in OK-VQA and validate the method with two KB-VQA benchmarks. The experimental results show that models can be improved significantly after incorporating the generated knowledge and our method is consistently helpful for different models for the final answer generation.
\item We conduct fine-grained analysis about the generated knowledge proving it is essential and faithful, which enhances the interpretability.
\end{enumerate}

\begin{table*}[t]
\centering
\begin{small}
  \begin{tabular}{lp{1cm}p{1cm}cc}
    \toprule
    \textbf{Model} & \textbf{Num. Shots} & \textbf{Extra Training} & \textbf{Explicit Knowledge} & \textbf{OK-VQA}\\
    \midrule
     \multicolumn{5}{c}{\textit{Few-shot Models}}\\ 
    PICa$_\text{175B}$&1 & \usym{2717}& \usym{2717} (GPT-3)& 36.4 \\ 
    PICa$_\text{175B}$&4 & \usym{2717}&\usym{2717} (GPT-3) & 43.3 \\ 
    PICa$_\text{175B}$&16 & \usym{2717}& \usym{2717} (GPT-3)& 46.5\\ 
    PromptCap$_\text{175B}$ & 1& \usym{2713}&\usym{2717} (OPT)&48.7\\ 
    PromptCap$_\text{175B}$ & 4&\usym{2713} & \usym{2717} (OPT)& 53.3\\ 
    PromptCap$_\text{175B}$ & 32& \usym{2713}&\usym{2717} (OPT) &60.4 \\ 
    \midrule
    \multicolumn{5}{c}{\textit{Zero-shot Models with Extra Training}}\\ 
    VL-T5$_\text{no-vqa}$& 0&\usym{2713} & \usym{2717} (T5)& 5.8\\  
    Frozen$_\text{7B}$ & 0&\usym{2713} &\usym{2717} (GPT-2)& 5.9\\ 
    VLKD$_\text{ViT-B/16}$& 0&\usym{2713} & \usym{2717}&10.5 \\ 
    VLKD$_\text{ViT-L/14}$& 0&\usym{2713} &\usym{2717} &13.6\\
    FewVLM$_\text{base}$& 0& \usym{2713}& \usym{2717}& 11.6 \\ 
    FewVLM$_\text{large}$& 0&\usym{2713} & \usym{2717}& 16.5\\ 
    BLIP-2(ViT-G+OPT)$_\text{7.8B}$ &0 & \usym{2713}&\usym{2717} (OPT)& 36.4 \\ 
    BLIP-2(ViT-G+FlanT5)$_\text{4.1B}$ & 0&\usym{2713} &\usym{2717} (FlanT5)&40.7 \\ 
    BLIP-2(ViT-G+FlanT5)$_\text{12.1B}$ &0 &\usym{2713} & \usym{2717} (FlanT5)& 45.9 \\ 
    Flamingo$_\text{3B}$ & 0& \usym{2713}& \usym{2717} (Chinchilla)&41.2\\ 
    Flamingo$_\text{9B}$ & 0&\usym{2713} &\usym{2717} (Chinchilla)& 44.7\\ 
    Flamingo$_\text{80B}$ &0 &\usym{2713} &\usym{2717} (Chinchilla) &50.6\\ 
    \midrule
    \multicolumn{5}{c}{\textit{Zero-shot Models \textbf{withou} Extra Training}}\\ 
    PICa$_\text{175B}$&0 &\usym{2717} &\usym{2717} (GPT-3)&17.7\\ 
    %PNP-VQA$_\text{3B}$(30Cap) &0 &\usym{2717} &T5 (implicit) & 31.4& \\ 
    %PNP-VQA$_\text{3B}$(50Cap) & 0&\usym{2717} &T5 (implicit) & 32.2& \\ 
    PNP-VQA$_\text{3B}$ & 0& \usym{2717}&\usym{2717} (T5)&34.1 \\ 
    PNP-VQA$_\text{11B}$& 0& \usym{2717}&\usym{2717} (T5)&35.9 \\ 
    Img2LLM$_\text{6.7B}$\footnote{for the result of 6.7B model, we re-run the model according to the provided code from the authors.} &30 syn. & \usym{2717}& \usym{2717} (OPT)&35.0 \\ 
    Img2LLM$_\text{13B}$ &30 syn. &\usym{2717} &\usym{2717} (OPT) &39.9 \\ 
    Img2LLM$_\text{13B}$ &15 syn. &\usym{2717} &\usym{2717} (OPT) & 37.0 \\ 
    Img2LLM$_\text{13B}$+KB-Gen &15 syn. &\usym{2717} &\usym{2717} (OPT) & 40.0 \\ 
    Img2LLM$_\text{30B}$ &30 syn. &\usym{2717} &OPT &41.8 \\ 
    Img2LLM$_\text{30B}$ &6 syn.&\usym{2717} &OPT &37.7 \\
    Img2LLM$_\text{30B}$+KB-Gen &6 syn.&\usym{2717} &OPT &42.2  \\ 
    %Img2LLM$_\text{30B}$ &0 &\usym{2717} &OPT (implicit) &41.8 &36.9 \\ 
    %Img2LLM$_\text{66B}$ &0 & \usym{2717}& OPT (implicit)&43.2 & 38.7\\ 
    Img2LLM$_\text{175B}$ &30 syn. & \usym{2717}&\usym{2717} (OPT)&45.6 \\ 
    KB-Gen$_\text{770M}$&0 &\usym{2717} &\color{green} \usym{2713} (GPT-3) &36.3\\
    KB-Gen$_\text{3B}$&0 &\usym{2717} &\color{green} \usym{2713} (GPT-3) &41.1 \\
    KB-Gen$_\text{11B}$&0 &\usym{2717} &\color{green} \usym{2713} (GPT-3) & \\
    \midrule
\end{tabular}
\end{small}
\caption{Comparison of model performances on OK-VQA dataset with different training strategies and knowledge sources. The first block of models require few training instances, the second block of models require no training instances but extra end-to-end training from other data sources rather than KB-VQA data, the last block of models are zero-shot models requiring no additional training.}
  \label{tab:main_results}
\end{table*}

%\midrule
%    \multicolumn{4}{c}{\textit{UnifiedQA FiE Model}}\\ 
%    \multirow{2}{*}{0.7B} 
 %    &\textit{w/o} Gen &  &\\
  %   &\textit{w} Gen &  &\\
   %  \cmidrule{2-4}
    % \multirow{2}{*}{3B} 
    % &\textit{w/o} Gen & 28.1 &\\
    % &\textit{w} Gen & 32.8 &\\

==> sections/related_v1.tex <==
\section{Related Work}
\label{sec:related}

% Knowledge-based VQA. One way to group related work is the source of knowledge: (1) methods using external structured knowledge bases, (2) recent methods using GPT-3 for knowledge. Another way to group related work is the use of training data: (1) methods relying on supervised training, (2) methods using pre-trained models (including models that can perform text-based QA such as UnifiedQA) and zero-shot or few-shot learning.

% Knowledge generation for text-based QA.

\subsection{Knowledge-based VQA}
Questions of Knowledge-based VQA (K-VQA) requires external knowledge beyond information from the image~\cite{DBLP:conf/cvpr/MarinoRFM19,DBLP:conf/eccv/SchwenkKCMM22,DBLP:journals/pami/WangWSDH18}. One line of works for K-VQA learn to retrieve relevant knowledge to questions from external knowledge bases~\cite{DBLP:journals/pami/WangWSDH18,DBLP:conf/eccv/NarasimhanS18,DBLP:conf/nips/NarasimhanLS18,DBLP:conf/mm/Li0020}, with K-VQA data. With the recently developed large language models (LLMs)~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20,DBLP:journals/jmlr/RaffelSRLNMZLL20}, which has been pre-trained with large data corpus, people convert visual question answering into a text-based question answering problem and leverage LLMs as implicit knowledge bases to obtain the answer~\cite{DBLP:conf/aaai/YangGW0L0W22,DBLP:journals/corr/abs-2211-09699,DBLP:journals/corr/abs-2212-10846}. Though good performance can be achieved, this line of work lack interpretability and it is unclear what external knowledge has been used for predicting answers. In this work, we try to bridge the research gap that we explicitly generate knowledge with LLMs first and explore whether the generated knowledge can facilitate K-VQA models.

\subsection{Knowledge Generation for Knowledge-intensive Tasks}
Knowledge-intensive tasks, such as commonsense question answering~\cite{DBLP:conf/nips/TalmorYBBGCB21} and open-domain question answering~\cite{DBLP:journals/tacl/KwiatkowskiPRCP19}, are in need of accessing external knowledge. Previous studies found augmenting models with retrieved knowledge conditioning on LLMs will improve model performance~\cite{DBLP:conf/nips/LewisPPPKGKLYR020,DBLP:journals/corr/abs-2208-03299}. Instead of retrieving knowledge, some of recent studies consider LLMs as abundant knowledge sources and directly generate relevant knowledge with LLMs~\cite{DBLP:journals/corr/abs-2210-01296,DBLP:journals/corr/abs-2209-10063,DBLP:conf/acl/0010LLWWBCH22}. They prompt LLMs (i.e., GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20}) with a few in-context examples and expect LLMs to generated knowledge in need for question answering. The good performances with the generated knowledge indicate that LLMs can be flexible knowledge sources to improve both the performance and intepretability of knowledge-intensive tasks. In this study, we intend to study whether knowledge generated from LLMs can benefit multimodal knowledge-intensive tasks, specifically, knowledge-based VQA.
